Diagnosing and Remedying Knowledge Deficiencies in LLMs via Label-free Curricular Meaningful Learning

Large Language Models (LLMs) are versatile and demonstrate impressive generalization ability by mining and learning information from extensive unlabeled text. However, they still exhibit reasoning mistakes, often stemming from knowledge deficiencies, which can affect their trustworthiness and reliability. Although users can provide diverse and comprehensive queries, obtaining sufficient and effective feedback is demanding. Furthermore, evaluating LLMs comprehensively with limited labeled samples is difficult. This makes it a challenge to diagnose and remedy the deficiencies of LLMs through rich label-free user queries. To tackle this challenge, we propose a label-free curricular meaningful learning framework (LaMer). LaMer first employs relative entropy to automatically diagnose and quantify the knowledge deficiencies of LLMs in a label-free setting. Next, to remedy the diagnosed knowledge deficiencies, we apply curricular meaningful learning: first, we adopt meaningful learning to adaptively synthesize augmentation data according to the severity of the deficiencies, and then design a curricular deficiency remedy strategy to remedy the knowledge deficiencies of LLMs progressively. Experiments show that LaMer efficiently and effectively diagnoses and remedies knowledge deficiencies in LLMs, improving various LLMs across seven out-of-distribution (OOD) reasoning and language understanding benchmarks, achieving comparable results to baselines with just 40\% training data. LaMer even surpasses methods that rely on labeled datasets for deficiency diagnosis. In application, our label-free method can offer an effective knowledge deficiency diagnostic tool for efficient LLM development.

==> chapters/2_preliminary.tex <==
\section{Preliminaries}
In this section, we first introduce the calculation of relative entropy when providing knowledge to LLMs. Next, we design an experiment to validate the feasibility of relative entropy by comparing it to other methods on the effectiveness of finding error examples.

\subsection{Relative Entropy of Knowledge}
\label{sec:re}
Relative entropy, also known as Kullback-Leibler divergence, can estimate the extra information needed to change form a distribution to another distribution~\cite{kullback1951information}, which is a quantitative measure of information volume. Thus, we can utilize relative entropy to estimate the information volume brought by knowlege.

Specifically, given a query $d$, which possesses a question $x$ and $n$ options $Y = \{y_1,y_2,\cdots,y_n\}$. We first send $d$ to LLM $\mathcal{L}$ to compute the probality of each option $y_i$ conditioned on $x$ and $Y$. Hereafter, we obtain a confidence distribution of $\mathcal{L}$ over $Y$:
\begin{equation}
\label{eq:p}
\begin{aligned}
    p_i &= \mathcal{L}(y_i|x,Y), \\
    P &= \text{Softmax}([p1, \cdots, p_n]),
\end{aligned}
\end{equation}
where $p_i$ denotes the prior probability of option $y_i$ conditioned on $x$ and $Y$ according to $\mathcal{L}$. $P\in\mathbb{R}^n$ denotes the prior confidence distribution of $\mathcal{L}$ on $\mathcal{Y}$. Softmax is the normalization function.

Secondly, we retrieve a piece of knowledge $k$ for $d$, then we introduce $k$ together with $d$ and $Y$ into $L$ to acquire a knowledge-based confidence distribution of $\mathcal{L}$ over $Y$:
\begin{equation}
\label{eq:q}
\begin{aligned}
    q_i &= \mathcal{L}(y_i|k,x,Y), \\
    Q &= \text{Softmax}([p1, \cdots, p_n]),
\end{aligned}
\end{equation}
where $q_i$ denotes the postrior probability of option $y_i$ after introducing $k$ to $\mathcal{L}$. $Q\in\mathbb{R}^n$ denotes the knowledge-based postrior confidence distribution of $L$ on $\mathcal{Y}$.

Finally, we can compute the relative entropy $\text{RE}$ with $P$ and $Q$ to quantify the difficiency of LLM $\mathcal{L}$ on $k$:
\begin{equation}
\label{eq:re}
    \text{RE} = -\sum_{i=0}^mp_i\times (log(q_i) - log(p_i)).
\end{equation}

Finally, we can consider the knowledge $k$ whoes $\text{RE}^j$ exceeds a threshold $\tau$ as a difficiency of $\mathcal{L}$.

\begin{table}[t]
\caption{Effectiveness of different methods on detecting difficiencies of Mistral~\cite{jiang2023mistral} based on e-CARE~\cite{du2022care}}
\centering
\tabcolsep=5.8pt
\begin{tabular}{lcccc}
\toprule
\textbf{Method}  & \textbf{Label Free} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    \\ \midrule
Golden Label     & \cellcolor[HTML]{FFCCC9}No       & 100       & 100    & 100   \\
Perplexity       & \cellcolor[HTML]{FFCCC9}No       & 48.46     & 34.24  & 40.10 \\
Random           & \cellcolor[HTML]{9AFF99}Yes        & 35.23     & 35.23  & 35.23 \\
Relative Entropy & \cellcolor[HTML]{9AFF99}Yes        & 40.34     & 64.30  & 49.58 \\ \bottomrule
\end{tabular}
\label{tab:preliminary}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/method.pdf}
    \caption{The whole workflow of Retro to automatically detect and alleviate the knowledge deficiencies of LLMs.}
    \Description{The framework of our proposed method.}
    \label{fig:method}
\end{figure*}


\subsection{Effectiveness of Detecting Difficiencies}
We conduct an inital experiment to reveal the effectiveness of different methods on finding difficiencies based on Mistral-7B-Instruct-v0.2~\cite{jiang2023mistral} and e-CARE~\cite{du2022care}. Implementation details can refer to Appendix~\ref{app:preliminary}. Results are shown in Table~\ref{tab:preliminary}, we can have the conclusions: even perplexity method adopts labels to indetify deficiencies, our proposed relative entropy method significantly outperforms the perplexity method by recalling more difficiencies for the specific LLM. This proves the superiority and feasibility of our proposed relative entropy method from the experimental point of view.



